Federated Learning and AI Regulation in the European Union: Who is Responsible? -- An Interdisciplinary Analysis

The European Union Artificial Intelligence Act mandates clear stakeholder responsibilities in developing and deploying machine learning applications to avoid substantial fines, prioritizing private and secure data processing with data remaining at its origin. Federated Learning (FL) enables the training of generative AI Models across data siloes, sharing only model parameters while improving data security. Since FL is a cooperative learning paradigm, clients and servers naturally share legal responsibility in the FL pipeline. Our work contributes to clarifying the roles of both parties, explains strategies for shifting responsibilities to the server operator, and points out open technical challenges that we must solve to improve FL's practical applicability under the EU AI Act.

==> chapters/archive/02_fl_workflow_stakeholders.tex <==





==> chapters/archive/03_liability_question.tex <==
Against this background, the responsibilities for the individual processes in the life cycle can be defined. While the classification under data protection law can be based on reasonably reliable findings, the assessment under the AI Act is still quite open.

\subsection{The “Easy” Part: FL under the GDPR}
The starting point for any data protection assessment of the processing of personal information is the question of the data controller responsible for each distinct phase of the data processing. The qualification as data controller comes with a variety of legal obligations towards the data subjects. In particular, the controller is obliged, inter alia, to comply with the data protection principles of lawfulness, fairness, transparency, purpose limitation, data minimization, accuracy, storage limitation, integrity and confidentiality of the processing of personal data (Art. 5 para. 1 GDPR). The controller is also accountable and must demonstrate compliance with the aforementioned requirements (Art. 5 para. 2 GDPR). 

Pursuant to Art. 4 para. 1 no. 7 GDPR, the controller is the person who alone or jointly with others decides on the purposes and means of the processing of personal data. The decision on "purposes" and "means" can also be understood as a decision on the "why" and "how" of processing. In addition to a sole responsibility for a particular data processing and a joint controllership (Art. 26 GDRP), actors in the FL lifecycle could also be classified as a processor pursuant to Art. 28 GDPR if they carry out data processing on behalf of a controller.

It appears that, on the one hand, the client involved in an FL lifecycle regularly has sole responsibility for the data acquisition and the data storage, as the FL server has no influence on these processes. On the other hand, the sole responsibility of the server for the processing of personal data for the purpose of validating the models and other model post-processing activities using personal information also seems quite clear. In contrast, the assessment of responsibility for the decentralized training of the models and for any personal data contained in the models  is not clear at all. In the context of conventional AI systems, the responsibility for this lies with the providers of the systems. This is doubtful in the case of FL, as the federated models are trained and maintained separately by the clients.

Correctly, the responsibility under data protection law should depend on the physical, technical and legal possibilities of the server to influence the model training and the configuration of the models. If, for example, the server retains control over the code that is run on the clients within the framework of a trusted execution environment (TEE) and the clients thus practically only have the authority to decide which data is used to train the model on their computers, it seems reasonable to assume joint controllership within the meaning of Art. 26 GDPR or - in the case of even more extensive binding of the clients - only a processing on behalf of the FL server within the meaning of Art. 28 GDPR. In any case, FL server and FL clients would have to enter into agreements (in the form of binding contracts) under both Art. 26 para. 1 GDPR and Art. 28 para. 2 GDPR, in order to determine their respective responsibilities for compliance with the obligations under the GDPR, in particular as regards the exercising of the rights of the data subjects (e.g. their rights to rectification and erasure under Articles 16 and 17 GDPR) and their respective duties to provide the information referred to in Articles 13 and 14 GDPR.

\subsection{The (More) Tricky Part: FL under the AI Act}
In principle, the AI Act does not have a differentiated allocation of roles for separate processing phases comparable to the GDPR. It is based on the “classic” image of an AI system that is operated centrally by a (single) provider. The definition of the provider is set out in Art. 3 para. 3 AIA, providing that “‘provider’ means a natural or legal person, public authority, agency or other body that develops an AI system or a general-purpose AI model or that has an AI system or a general-purpose AI model developed and places it on the market or puts the AI system into service under its own name or trademark, whether for payment or free of charge”. Depending on the (high) risk area for which the system is designed, the AIA links a number of obligations to the provider role in Articles 8 et seq. AIA, in particular data and data governance obligations under Art. 10 AIA. 

At first glance and from a strictly technical perspective, both the FL server and the FL clients fall under the provider concept of Art. 3 para. 3 GDPR, as they are all involved - with individually different functions and independent purposes - in the development of the FL system. However, since the AI Act - unlike the GDPR - focuses less on responsibilities for individual, definable data processing processes and more on secure system design as a whole, the provider concept will have to be teleologically limited to the FL server if and to the extent that it is solely responsible to the outside world and offers the FL system on the market. A “joint providership” (based on “joint controllership” under the GDPR) does not exist under the AI Act.

This will certainly not make things any easier for the FL server. Unlike Art. 26 and 28 GDPR, Articles 8 et seq. AIA do not provide any details regarding the governance required in networked processing environments such as FL systems. In particular, Art. 10 AIA does not specify what precautions a FL server must take in order to fulfill its obligations under the AI Act. The only certainty appears to be at this point that it must take such precautions and is responsible for all processes in the FL lifecycle. 

It seems very realistic that this may have an impact on the data protection assessment of the FL lifecycle. If the FL server, in fulfillment of its obligations under the AEOI, in particular Art. 10 AEOI, sets far-reaching requirements for the FL clients with regard to the training of the models and the handling of the training data, these requirements could lead to the FL server being classified as a controller under data protection law within the meaning of Art. 4 para. 1 no. 7 GDPR, while the FL client is classified as a mere processor within the meaning of Art. 28 GDPR. 


==> chapters/archive/04_technical_implications.tex <==
Realistically, it is challenging to facilitate liability tracking in FL systems that learn from thousands of clients. 
While clients are legally required to report on lifecycle steps under their control, we must consider server-side solutions to take on this responsibility. 
Otherwise, the chances of opening up the client data silos will remain vanishingly small.
Therefore, we must design technical solutions that achieve the following: 

\textbf{Federated Data Auditing}. 
To establish a legally compliant FL lifecycle, the server must assume responsibility for the entirety of the training process. 
Thus, we require approaches allowing client-side data audits that can be shared with the server operator without infringing data protection. 
Interestingly, promising steps in this direction are coming from security research, specifically of membership inference \citep{Huang2023}. 
The goal is to establish a (synthetic) calibration dataset that can be used to assess the data quality or bias present in a client dataset. 
Yet, this clearly opens a potential attack vector since such methods allow inferring significant metadata about clients, which can yield data leakage.

\textbf{Trusted Execution}. 
To support server operators in establishing an audit-proof FL lifecycle, we require approaches that allow trusted execution at scale. 
Clients can use such TEEs to prove they are providing tampering-free model updates. 
Yet, with the emergence of generative AI models in FL, we require TEEs that either allow for encapsulation of entire processes that can consume multiple gigabytes of (GPU) memory and disk \cite{Raffel2019} or integrity proofs that can run in established TEE technology \cite{Muoz2023}.


